CARE: Content Aware Redundancy Elimination for Disaster Communications on Damaged Networks

During a disaster scenario, situational awareness information, such as location, physical status and images of the surrounding area, is essential for minimizing loss of life, injury, and property damage. Today's handhelds make it easy for people to gather data from within the disaster area in many formats, including text, images and video. Studies show that the extreme anxiety induced by disasters causes humans to create a substantial amount of repetitive and redundant content. Transporting this content outside the disaster zone can be problematic when the network infrastructure is disrupted by the disaster. This paper presents the design of a novel architecture called CARE (Content-Aware Redundancy Elimination) for better utilizing network resources in disaster-affected regions. Motivated by measurement-driven insights on redundancy patterns found in real-world disaster area photos, we demonstrate that CARE can detect the semantic similarity between photos in the networking layer, thus reducing redundant transfers and improving buffer utilization. Using DTN simulations, we explore the boundaries of the usefulness of deploying CARE on a damaged network, and show that CARE can reduce packet delivery times and drops, and enables 20-40% more unique information to reach the rescue teams outside the disaster area than when CARE is not deployed.

==> background.tex <==
\section{Background}

[[STILL WORKING ON THIS SECTION. IGNORE]]


SA information can include many things, such as location information (of fires, floods, damaged homes), the status of the disaster (e.g., temperature of a fire, water levels in a flood, direction of movement of flood or fire), resource information (such as rescue, medical, water and food resources), and the status of individuals (e.g., health monitoring, distress calls). 

People's everyday devices, such as smartphones, cameras, and laptops, enable ordinary citizens (i.e., not just first responders) inside a disaster zone to gather critical information in a variety of formats, including text, photos, audio and video. In the near future handheld devices will also contain sensors, such as pollution, temperature, and humidity, that will only further enrich a person's ability to gather timely SA information.
In fact, today's handhelds almost make it too easy for ``humans as sensors" \cite{camas} to gather data which can lead to information overload that complicates rapid decision making.
Eyewitness accounts on the ground can be surprisingly helpful when the usual mechanisms for SA data gathering are hindered by the disaster itself. For example, during the Pakistan floods in 2010, Google said ``Although we've been able to provide satellite imagery for disasters in the past, cloud cover in Pakistan has prevented us from compiling useful imagery so far. \cite{google-pakistan}"

% Google actually solicited map data from those on the ground.


Recently we have witnessed an upsurge in the use of online social networks, such as Twitter \cite{twitter-use-09} and Facebook \cite{facebook-use-08}, as well as the emergence of new Web-based applications that can both assist victims, and enable ordinary citizens to involve themselves in the emergency response effort. An an example of these applications is Ushahidi \cite{ushahidi} that allows individuals to upload text and photos that are aggregated and displayed either as a list of reports or on a Google map. A second example is Google's PeopleFinder \cite{people-finder} that allows those outside the disaster zone to try to locate loved ones inside the disaster zone. Studies have shown that, when citizens in a disaster area have Internet connectivity, they are very willing to contribute to SA by sharing photos \cite{photo-sharing}, micro-blogging \cite{twitter-use-09}, and to engage in collective problem solving, e.g., figuring out lists of victims during an incident \cite{facebook-use-08}.



We believe that it is important to work on the infrastructure problems underlying these new applications which have seen a burst in activity due in part to a calamitous year in 2010. According to \cite{badyear2010}, ``earthquakes, heat waves, floods, volcanoes, super typhoons, blizzards, landslides and droughts killed at least a quarter million people in 2010." Climate scientists say that due to global warming, natural disasters are on the rise.  The use of the web to provide SA during disasters is a trend that is likely to continue to gain momentum. For example, two out of Twitter's top 10 overall trends in 2010 (\cite{TwitterTrends}), were on topics about disasters (The Gulf Oil Spill and Haiti).  Moreover, a rich offering of crisis response software is around the corner, as evidenced by efforts such the as ``Random Hacks of Kindness Hackathons" \cite{hackathon} that bring together volunteer programmers and experts in disaster response for two-day events to create software solutions focused on disaster response. Other efforts include the development of data formats for crisis response data \cite{google-data-formats}, the development of visualization techniques \cite{mashups}, and the ongoing development of new applications and portals for these applications \cite{portal-iscram08}.




==> discussion.tex <==
\section{Discussion}


In this study we have focused on the redundancy of semantic content in photos. We believe that the framework we are proposing here could be applied to other media types as well. Our approach could also be applied to text data in which the computer vision techniques are replaced by natural language processing techniques to identify semantic redundancy.
Although the study in \cite{tretweet} did a qualitative analysis of redundant content in twitter discussions about disasters, they did not quantify the amount of redundancy from the point of view of messages that could potentially be dropped to alleviate congestion. To illustrate the potential of our approach to text, we analyzed the pager message dataset from the 9/11 attack. This data was collected from multiple providers in and around Manhattan on September 11 from 3 am until 3 am the following day, and was made publicly available by one of the providers for a short period of time in 2009. Using natural language processing methods and a decision-tree classifier, we managed to classify over 55\% of the messages using 6 situational awareness classes. This classification enables identifying similar text messages, and by using aggregation methods,
e.g., instead of sending all messages we send only the class identification and the list of senders,
we believe it is possible to achieve significant traffic reduction. We leave this study for future research.


\ignore{
messages to belong to specific classes and aggregate the messages that belong to each class.

There are a number of ways to potentially quantify the amount of redundancy in text messages. For this initial evaluation, we used a 3 step method. First, we classify messages into specific classes using NLP methods (such as Decision Trees and Naive Bayes). We used 6 classes, namely: 1. \textbf{Seeking help} 2. \textbf{Offering help} 3.
\textbf{I am okay} 4. \textbf{Are you okay?} 5. \textbf{Situational Awareness} and 6. \textbf{Others} where {\bf Other} messages are those unrelated to the disaster. The second step is to use aggregation policies to create a single representative message of those in a group, thereby sending only one message for the group within a window of time. For example, to aggregate ``I'm ok" messages one could send a single message with a list of all the people who are ok. The third step involves the use of a forwarding policy. For example, one could forward all original messages as is, and only drop the ``Other" messages. In the 911 dataset, this resulted in a content reduction of roughly 55\% because there are many messages in the dataset that are unrelated to the world trade center event (e.g. such as system update messages). An alternate policy would be to forward the ``other" messages, if they are viewed as too ambiguous to be handled by classification, and then send only one aggregated message per class (within a given time window). This resulted in a 45\% reduction in dataset size for this pager data. These calculations indicate that for such datasets there is a potential to cut in half, roughly, the amount of messages that need to cross a network. As future work, we intend to explore the issues around identifying and reducing content redundancy in text messages in the context of disaster events.
}


%We used methods from Natural Language Processing to classify messages to belong to specific classes and aggregate the messages that belong to each class.

%We observed that messages can belong to one of the following six classes:
%\begin{itemize}
% \item \textbf{Seeking help}:  Messages originating from the victims asking for help. The messages that belong to this class can be aggregated by sending the list of sender geo-locations.
% \item \textbf{Providing help}: Messages from the first responders advertising support and help. These messages can be combined by sending the list of sender phone numbers.
% \item \textbf{I am okay:} Messages from survivors informing their friends and relatives that they are okay. We can aggregate the messages here to send the list of sender phone  numbers.
% \item \textbf{Are you okay?:} Messages from anxious friends and relatives enquiring if the recepient is fine in the wake of the disaster. These messages can be aggregated by sending a list of sender, receiver phone number tuples.
% \item \textbf{Situational Awareness:} Messages that describe the scenario in the region inflicted by the disaster. Clustering techniques can be applied on these text messages to identify the different topics and sample messages related to each topic can be sent.
% \item \textbf{Others:} Messages that are not related to disasters. We observed several machine-generated text messages. These can be either ignored or have to be sent completely depending on the network capacity.
%\end{itemize}



==> motivation.tex <==
\section{Redundancy in Data}

In this section we motivate the use of a content-aware approach to information overload in disasters. We describe the datasets we worked with, the difficulties involved with defining ``similarity" for pairs of images and groups of text messages, and how we evaluated the amount of semantic redundancy in each. These dataset evaluations serve as illustrations of the kinds of semantic redundancy that can occur, and confirm our the intuition and anecdotes around redundancy in traffic that occurs during disasters.

\subsection{Image Data}
\label{sec:image_redundancy}

We used two datasets of photographs for our study on image redundancy. The first dataset, labeled {\em SDfire}, was obtained from the San Diego fire in 2007 \cite{karl}. This dataset contains 84 pictures taken by a professional photographer who wandered around one of the affected towns both during the fire event and afterwards.  The pictures depict a variety of scenes including burning homes, damaged homes and cars, firefighters, policemen, etc. This dataset serves as one example of the kind of data, and data redundancy, that could be generated by a single individual.

The second dataset, labeled {\em Haiti}, was obtained through the generosity of an organization called Team Rubicon \cite{TeamRubicon}. Team Rubicon sends small teams, of roughly 10 people that are primarily medical staff, into disaster zones. They set up temporary huts where they administer medical emergency services. Their teams often move from one day to the next, to reconstruct their service station in different parts of the affect area. Team Rubicon gave us their photos that were taken by one such team during the Haiti earthquake in January 2010. The photos are a collection from a number of people on the team, including the doctors, their organizational personnel and one professional photographer. Their photos cover a wide range of subjects including wounded people, damaged buildings, rescue vehicles (jeeps, helicopters), victims trapped under ruble, the medical staff, the service stations, street scenes, famous buildings, and crowd formations of victims. This dataset contains 415 images.

In both of these datasets, it was clear to us, just by casually perusing the data, that there were plenty of pairs of images that were similar. We also saw instances of 3 photos, or even 4 photos that were clearly similar, to an untrained eye. However, before even starting to think about how to detect semantic redundancy in an automated fashion, we need to define a notion of ground truth; that is, to establish a way to quantify the redundancy in these datasets, so that later on we can understand the target amount of redundancy an automated algorithm can be expected to detect. We decided to label the data ourselves, by hand, and built a tool to facilitate the labeling procedure via visual aids. Our tool lets the labeler view two images at a time and allows him to rate the similarity of the two images on a scale from 0 to 5, where 0 means not similar at all, and 5 means extremely similar. [[Should we try to justify the choice of 0 to 5 by claiming we were inspired by the Likhert scale ??]]

%% TBD -- "luminances" (plural form) is correct spelling?
The notion of "similarity" is a difficult one to define precisely. Some cases are straightforward such as examples of two photos of exactly the same scene in which a) one image is in focus and the second is not; b) two photos with different luminance; or c) the two photos have different resolution. However, consider a more complicated example. Suppose photos A and B contain the same person in 2 different background scenes (let's say 2 different places on the same block), and this person appears ok in his health. If the goal of the situational awareness application is merely to find people, or to report whether or not people are ok, then these two images can be considered redundant. However if the goal of the application is to track a person's movements, then the two photos are not redundant. Moreover if the background information contains a burning house in one image and not in the other, and the application aims to understand where help is needed, then these two images are clearly not redundant. It becomes clear that the notion of similarity is subjective, and more importantly, ultimately depends upon the "intended use" of the data. Recall that our focus is on situational awareness applications, and the goal of such applications typically include things such as enabling victims in the field to get the status of what is happening in a given location, or for rescue workers to know which houses are on fire or not, or to know in which locations help is available, and so on.

Because the notion of similarity is hard to specify precisely, even for manual labeling, we decided to consult with experts that have experience in disaster events. We worked with members of our city's Disaster and Fire Commission, and the local Amateur Ham Radio Club \cite{fire-commission}, who have experience helping in local neighborhoods during fire and earthquake events. In addition to advising us on what might be considered "similar" by first responders, they also kindly agreed to use our labeling tool and do the labeling for us.

% TBD -- what is sketching? do you mean stitching?
% -- check the numbers - I think it's the other way around, no?
Given the data labels, we measure the amount of redundancy as follows. The goal of our system is for devices to detect redundancy in two images. Once this redundancy has been detected, the forwarding device has a few options for reducing the amount of traffic. One is to simply send only of the two images and to drop the second. Another option is to put one of the images at the back of the priority queue and only send it, if and when sufficient bandwidth becomes available. A third option is to combine images via techniques such as sketching \cite{}. In this work, we focus on the first option. Therefore we can quantify the amount of redundancy using a set cover notion. If a subset $s$ of photos, is comprised of $n$ similar images, then it is sufficient to send a single image to cover (or represent) that subset. If we let $S$ denote the complete set of photos, then our goal is to find the minimum subset of photos so that the entire set $S$ would be represented. In other words, ideally our routers would send the minimum amount of photos to convey all the information in the entire dataset. Using this definition and our labeled data, we found that the {\em SDfire} data has 53\% redundancy, and the {\em Haiti} dataset has 22\% redundancy. This means that sending less than half the photos in the {\em SDfire} data, we convey all of the unique information.

We point out that this way of quantifying redundancy yields a quantity that may be unattainable in a real network. We can compute the minimum set cover on our dataset because we have the entire dataset on hand. When such data is generated by multiple people scattered over a disaster zone, it is most likely that each forwarding devices will only ever see a portion of this data. Each device can only detect and remove the redundancy that travels through it. Hence this quantification of redundancy serve as an optimal upper bound on the amount of potential redundancy to be detected and eliminated inside a network.


\subsection{Text Data}
\textbf{XX Transistion paragraph XX}

\textbf{XX TBD - some of this should go to related work.}
Previous research has shown the prevalence of text-based communication during disasters \cite{tmassconv, tmicroblog, siteseeing}. \textbf{XX More details here? XX}Studies have also shown that there is a large amount of redundancy in the text-based messages related to disasters \cite{tretweet}. We use techniques from Natural Language Processing to identify text messages that are similar at a semantic level and describe possible ways of aggregating the messages to eliminate semantic level redundancy. %Our study is based on two media of communication that are widely used during a disaster scenario namely text messaging and communication over social networks (Twitter).

\textbf{XX Source XX} We use the pager message dataset from the 9/11 attack, labelled {\em WTC} to study the redundancy in text messages during a disaster. The {\em WTC} dataset consists of 448376 pager messages that were intercepted in and around Manhattan on September 11 from 3 am on the same day till 3 am the following day, covering the complete 24 hours surrounding the 9/11 attacks. We see that there is a sharp surge in the message rate at about 9 am, shortly after the first tower was hit with a peak rate of 1000 messages per minute.

\textbf{XX TBD - perusing XX}
After perusing the messages in the dataset, we identified patterns in the pager messages in the dataset. Previous research~\cite{siteseeing} has also shown similar trends in messages from disaster areas.
\textbf{XX Move Others to the class XX}

\textbf{XX Talk about aggregation ahead and add hereXX}
Our first observation was the presence of a large percentage of messages that were machine generated messages and that are not related to the disaster itself. %A sample message of this kind is:
% {\em root@avm1.scc911.com|avm1|user processes are taking up a large percentage of cpu. login and use top to see if there is a problem.}
We also observed a small fraction of human-generated messages that were not related to the disaster. These messages that are not related to the disaster (both human-generated and machine-generated) are not of interest to us and we label them as {\em Other messages}.


The messages that were related to the disaster fitted into one of the following five broad classifications:
\begin{itemize}
\item \textbf{Seeking help:} Messages originating from the victims asking for help.
\item \textbf{Providing help:} Messages from the first responders advertising support and help.
\item \textbf{I am okay:} Messages from survivors informing their friends and relatives that they are okay.
\item \textbf{Are you okay?:} Messages from anxious friends and relatives enquiring if the recepient is fine in the wake of the disaster.
\item \textbf{Situational Awareness:} Messages that describe the scenario in the region inflicted by the disaster.
\end{itemize}

We perform pre-processing on the messages before applying various Natural Language Processing techniques. First of all, we filter out short functional words such as  {\em the, is, at, on} etc from the messages. These words are called {\em stop words} and they contain low information content as opposed to the key words in the message. We use the English stopword corpus in the Natural Language Tool Kit (NLTK) package \cite{NLTK} for this step. We also perform {\em Stemming} on the words in the message. Stemming is the process of reducing inflected words to their base form. For example, running will be reduced to run. We use the Porter Stemming Algorithm to perform this task.

In order to perform classification of the text messages, we need to extract features from the pre-processed message. We apply the {\em Bag of Words} model to extract the features. In this model, the text is represented as the unordered collection of words that comprise it.

The features extracted using the bag of word technique is given as input to the various classification techniques. We used the Na\"ive Bayes classification algorithm and the Decision Tree algorithm to clasify the text messages into one of the six categories mentioned above (including the Other message category). The Na\"ive Bayes approach uses prior probabilities of each class and the contribution from each word to estimate the likely class. The decision tree algorithm builds a flowchart on the features and uses this flowchart and the features in the message to classify it.

We manually labelled 1000 text messages to belong to one of the six classes. We conducted tests on these labelled messages by varying the training and test set size and found that the two approaches have different trade-offs. A few sample points can be found in Table~\ref{tab:naive}. We see that the Na\"ive Bayes approach has higher recall and lower precision. The Decision Tree classifiers show higher precision but lower recall. Note that the precision and the recall values are averaged over the five classes representing messages related to disasters. The apt algorithm and the right operating point can be chosen based on the aggregation strategy.

\begin{table}
\begin{center}
\begin{tabular} {| c | c | c || c | c |}
\hline
 & \multicolumn{2}{|c|}{Na\"ive Bayes} & \multicolumn{2}{|c|}{Decision Tree}\\
\hline
Training Size & Precision  & Recall & Precision & Recall \\
\hline
500 & 0.56 & 0.96 & 0.91 & 0.83\\
700 & 0.63 & 0.95 & 0.88 & 0.83\\
800 & 0.62 & 0.97 & 0.90 & 0.84\\
\hline
\end{tabular}
\caption{\textbf{XX Change to FP and FN XX} Precision and Recall for Na\"ive Bayes algorithm on the 1000 labelled messages for different training set sizes}
\vspace{-0.3in}
\label{tab:naive}
\end{center}
\end{table}

%\begin{table*}
%\begin{center}
%\begin{tabular} {| c | c |}
%\hline
%Class & Aggregation Strategy \\
%\hline
%Seeking help & List of sender geo-locations  \\
%Providing help & List of sender phone numbers \\
%I am okay & List of sender phone numbers \\
%Are you okay & List of sender phone number, receiver phone number tuples \\
%Situational Awareness & K-means Cluster centers \\
%\hline
%\end{tabular}
%\caption{Aggregation Strategy for various text message classes}
%\vspace{-0.2in}
%\label{tab:agg}
%\end{center}
%\end{table*}

\textbf{XX Move this para earlier XX} We can achieve content reduction by performing aggregation of the messages in each class. The aggregation strategy for should be able to summarize the important information that needs to be extracted from the messages belonging to that particular class. The set of aggregation strategies that we propose for each class can be found in Table~\ref{tab:agg}. Unlike the other classes, there is no key information that can be extracted from the messages from the situational awareness class. However there is high similarity in the messages in this class in terms of the key words used. Hence, we propose to perform K-means clustering algorithm on the message features and send a representative message for each cluster (point closest to the centers). For the messages, belonging to the Other messages class, we do not propose any aggregation strategy since the messages tend to be varied and unrelated.

\textbf{Results para}

The content reduction mechanism that we propose is highly flexible and we can achieve different levels of reduction based on the network conditions and the priorities of the classes driven by policy. A few sample policies and the amount of content reduction that we achieve is shown in Table~\ref{tab:policy}

%\begin{table*}
%\begin{center}
%\begin{tabular} {| c | c |}
%\hline
%Policy & Percentage Reduction \\
%\hline
%Send Other Messages, Aggregate rest &   \\
%Suppress Other Messages, Send rest &  \\
%Suppress Other Messages, Aggregate rest & \\
%\hline
%\end{tabular}
%\caption{Content Reduction Policies and the percentage content reduction achieved in the pager dataset}
%\label{tab:policy}
%\vspace{-0.2in}
%\end{center}
%\end{table*}

Based on the real world pager dataset, we see that there is a lot of redundancy at the semantic level in the messages from the disaster area leading to a huge potential in reduction of traffic. Semantic traffic reduction can not only reduce the traffic that traverse the damaged network, but also can help first responders and rescue operators parse through the huge surge of data coming in with ease.


 %   Description of the dataset

 %- Different classes of messages

 %- Classification techniques like Na\"ive Bayes and Decision Tress and precision/recall

 %- Aggregating the classes - Clustering etc

 %- Final numbers from the dataset.




%Twitter based study



     % Use text data as examples: 911 pager dataset, Arkansas floods event. Provide a measure of redundancy for these datasets based on the NLP techniques and a classification system.

